Integer Linear-Exponential Programming in NP by Quantifier Elimination

This paper provides an NP procedure that decides whether a linear-exponential system of constraints has an integer solution. Linear-exponential systems extend standard integer linear programs with exponential terms $2^x$ and remainder terms ${(x \bmod 2^y)}$. Our result implies that the existential theory of the structure $(\mathbb{N},0,1,+,2^{(\cdot)},V_2(\cdot,\cdot),\leq)$ has an NP-complete satisfiability problem, thus improving upon a recent EXPSPACE upper bound. This theory extends the existential fragment of Presburger arithmetic with the exponentiation function $x \mapsto 2^x$ and the binary predicate $V_2(x,y)$ that is true whenever $y \geq 1$ is the largest power of $2$ dividing $x$. Our procedure for solving linear-exponential systems uses the method of quantifier elimination. As a by-product, we modify the classical Gaussian variable elimination into a non-deterministic polynomial-time procedure for integer linear programming (or: existential Presburger arithmetic).

==> procedure-Bareiss-extended.tex <==
{%\addtolength{\textfloatsep}{-1in}
\begin{algorithm}[t]
  \caption{\ExtGaussianQE: Gauss--Jordan elimination for existential Presburger arithmetic.}
  \label{algo:gaussianqe-extended}
  \label{algo:extgaussianqe}
  \begin{algorithmic}[1]
	  \Require \hspace*{-0.5em}\begin{tabular}[t]{l}$\vec x:{}$ sequence of variables;\\$\phi^\circ(\vec x, \vec z) :{}$ Boolean combination of linear constraints without $<$.\end{tabular}
    \NDBranchOutput
      Boolean combination $\psi_\beta(\vec z)$ of linear constraints. %(in)equalities and divisibility constraints.
    \GlobalSpec
      $\bigvee_{\beta} \psi_\beta$ is equivalent to $\exists \vec x \,\phi^\circ$.
    \medskip
    %
    \State $\phi \gets \phi^1 \land \phi^2$ where:\newline{}
	   \mbox{}\quad $\phi^1 = \bigwedge (\tau + y_\tau = 0)$ over all inequalities $\tau\le 0$ and equalities $\tau=0$ in $\phi^\circ$,\newline{}
	   \mbox{}\quad $\phi^2$ is $\phi^\circ$ with each $\tau\le 0$ replaced by $y_\tau\ge 0$ and each $\tau=0$ by $y_\tau=0$,\newline{}
	   \mbox{}\quad where $y_\tau$ are fresh slack variables
           \label{extgauss:introduce-slack}
    \State $\lead \gets 1$; \quad
           $s \gets ()$ \label{extgauss:bareissfactors}
    \Comment{$s$ is an empty sequence of substitutions}
    %\Comment{lead coefficient}
    \ForEach{$x$ in $\vec x$} \label{extgauss:mainloop}
       \If{no equality of $\phi$ contains $x$} \mycontinue \EndIf \label{extgauss:triviality-check}
       \State \myguess $a x + \tau = 0 \ \text{(with $a \ne 0$)} \gets \text{equality in $\phi$ that contains $x$}$ \label{extgauss:guess-equation}
       \State $\prevlead \gets \lead$; \quad $\lead \gets a$
       \Comment{previous and current lead coefficients}
       \label{extgauss:new-factor}
       \If{$\tau$ contains a slack variable $y$ not assigned by $s$}\label{extgauss:branch}
	  \State \myguess $v \gets \text{integer in $[- |a| \cdot \fmod(\phi), + |a| \cdot \fmod(\phi)]$}$ \label{extgauss:guess-slack}
	  \State append $\sub{v}{y}$ to $s$ \label{extgauss:append-seq}
       \EndIf
       \State $\phi \gets \phi \vigsub{\frac{-\tau}{a}}{x}$ \label{extgauss:vig}\label{extgauss:vigorous}
       %\Comment{in inequalities, the sign is flipped if $a<0$} (already in the definition of ``vigorous'')
       \State divide each constraint in $\phi$ by \prevlead \label{extgauss:divide}
       \Comment{in divisibility constraints, both sides are affected}
       \Statex\Comment{in inequalities, the sign is flipped if $\prevlead<0$}
       \State $\phi \gets \phi \land (a \divides \tau)$ \label{extgauss:restore}
    \EndFor \label{extgauss:endmainloop}
    \ForEach{equality $\eta' + m y = 0$ of $\phi$ with some slack variable $y$ not assigned by $s$} \label{extgauss:unslackloop}
       \State %\textbf{let} $\eta$ be $\eta' + m y$ with $m \in \Z$;\quad
	      \textbf{if} $\eta'$ is different from $0$:\quad
              replace $m y$ with $-\eta'$ in $\phi$
	      \label{extgauss:drop-slack}
    \EndFor
    \State apply substitutions of $s$ to $\phi$ \label{extgauss:apply-seq}
    \ForEach{$x$ in $\vec x$ that occurs in $\phi$} \label{extgauss:loop-rem}
       \State \myguess $r \gets \text{integer in $[0, \fmod(\phi)-1]$}$ \label{extgauss:guess-rem}
       \State $\phi \gets \phi \sub{r}{x}$ \label{extgauss:subst-rem}
    \EndFor
    \State \textbf{return} $\phi$
  \end{algorithmic}
\end{algorithm}%
}%


==> procedure-IntegerWrapper.tex <==
\begin{algorithm}[t]
  \caption{\textsc{LinExpSAT[$\Z$]}: 
  An~\np procedure to decide linear-exponential systems over $\Z$.}
  \label{algo:wrapper-for-integers}
    \begin{algorithmic}[1]
      \Require
        $\varphi(x_1,...,x_n):{}$ linear-exponential system (without divisibility constraints).
      \Ensure
        \textbf{True}:{} if and only if $\varphi$ has a solution over $\Z$.
      \medskip
      \ForEach{equailty $(\tau = 0)$ in $\phi$}
        update $\phi$ : replace $(\tau = 0)$ by $(\tau \leq 0) \land (-\tau \leq 0)$
      \EndFor
      \State $I \gets{}$\textbf{guess} a subset of $[1,n]$ 
      \Comment{Assume $x_i \leq 0$ for all $i \in I$}
      \State $\phi \gets \phi\sub{0}{(x \bmod 2^{x_i}) :\text{$x$ is a variable and $i \in I$}}\sub{-x_i}{x_i : i \in I}\sub{2^{-x_i}}{2^{x_i} : i \in I}$
      \State \textbf{let} $z$ and $z_i$ (for every $i \in I$) be fresh variables
      \State $\psi \gets (z = \sum_{i \in I} x_i) \land \bigwedge_{i \in I} (z_i = \sum_{j \in I \setminus \{i \}} x_j)$
      %\Comment{if $I = \emptyset$ then $\psi$ 
      %  is $(z = 0)$}
      \Comment{$(\bigwedge_{j \in \emptyset} \cdot) \coloneqq \top$ and $(\sum_{j \in \emptyset} \cdot) \coloneqq 0$}
      \While{some term $-x_i$ with $i \in I$ occur exponentiated in $\phi$}
        \State \textbf{let} $\gamma \coloneqq (\tau \sim \sigma)$ be an (in)equality of $\phi$ such that 
        $\tau$ does not have terms $2^{-x}$,
        \Statex\hspace{1.8cm} 
          ${\sim} \in \{{<}\,,\,{\leq}\}$,\,
          $\sigma \coloneqq \sum_{i \in I} a_i \cdot 2^{-x_i}$ with some $a_i \neq 0$
          \State $b \gets \sum_{i \in I} \abs{a_i}$
          \State $g \gets{}$\textbf{guess in }$[-b,b] \cup \{\star\}$
          \If{$g = \star$} update $\phi$ : replace $\gamma$ by $(\tau < -b)$
          \Else
            \ update $\phi$ : replace $\gamma$ by $(\tau = g) \land (g \cdot 2^z \sim \sum_{i \in I} a_i \cdot 2^{z_i})$
          \EndIf
      \EndWhile
      \State\label{algo:wrapper-for-integers:call-to-N} \textbf{return }\Call{LinExpSAT[$\N$]}{$\phi \land \psi$}
    \end{algorithmic}
  \end{algorithm}
